Deciphering 'What' and 'Where' Visual Pathways from Spectral Clustering of Layer-Distributed Neural Representations

We present an approach for analyzing grouping information contained within a neural network's activations, permitting extraction of spatial layout and semantic segmentation from the behavior of large pre-trained vision models. Unlike prior work, our method conducts a holistic analysis of a network's activation state, leveraging features from all layers and obviating the need to guess which part of the model contains relevant information. Motivated by classic spectral clustering, we formulate this analysis in terms of an optimization objective involving a set of affinity matrices, each formed by comparing features within a different layer. Solving this optimization problem using gradient descent allows our technique to scale from single images to dataset-level analysis, including, in the latter, both intra- and inter-image relationships. Analyzing a pre-trained generative transformer provides insight into the computational strategy learned by such models. Equating affinity with key-query similarity across attention layers yields eigenvectors encoding scene spatial layout, whereas defining affinity by value vector similarity yields eigenvectors encoding object identity. This result suggests that key and query vectors coordinate attentional information flow according to spatial proximity (a `where' pathway), while value vectors refine a semantic category representation (a `what' pathway).

==> Makefile <==
# programs
LATEXMK  = latexmk
PDFLATEX = pdflatex -halt-on-error -interaction=nonstopmode --shell-escape
TOUCH    = touch
RM       = rm

# compilation targets
targets   := main
pdf_files := $(addsuffix .pdf,$(targets))

# intermediate files
d_files   := $(wildcard $(addsuffix .d,$(targets)))
aux_files := $(addsuffix .aux,$(targets))
bbl_files := $(addsuffix .bbl,$(targets))
blg_files := $(addsuffix .blg,$(targets))
brf_files := $(addsuffix .brf,$(targets))
log_files := $(addsuffix .log,$(targets))
fls_files := $(addsuffix .fls,$(targets))
fdb_files := $(addsuffix .fdb_latexmk,$(targets))
out_files := $(addsuffix .out,$(targets))

# default target
.PHONY: default
default: all

# all targets
.PHONY: all
all: $(pdf_files)

# build rules
$(pdf_files): %.pdf: %.tex
	@$(LATEXMK) -pdf -pdflatex="$(PDFLATEX)" -M -MF $*.d $*.tex;\
	 $(TOUCH) $*.pdf $*.d
ifneq ($(d_files),)
-include $(d_files)
endif

# clean
.PHONY: clean
clean:
	$(RM) -f\
            $(aux_files)\
            $(bbl_files)\
            $(blg_files)\
            $(brf_files)\
            $(log_files)\
            $(fls_files)\
            $(fdb_files)\
            $(out_files)\
            $(d_files)\
            $(pdf_files)

